Benchmarking Automated Clinical Language Simplification: Dataset, Algorithm, and Evaluation

Patients with low health literacy usually have difficulty understanding medical jargon and the complex structure of professional medical language. Although some studies are proposed to automatically translate expert language into layperson-understandable language, only a few of them focus on both accuracy and readability aspects simultaneously in the clinical domain. Thus, simplification of the clinical language is still a challenging task, but unfortunately, it is not yet fully addressed in previous work. To benchmark this task, we construct a new dataset named MedLane to support the development and evaluation of automated clinical language simplification approaches. Besides, we propose a new model called DECLARE that follows the human annotation procedure and achieves state-of-the-art performance compared with eight strong baselines. To fairly evaluate the performance, we also propose three specific evaluation metrics. Experimental results demonstrate the utility of the annotated MedLane dataset and the effectiveness of the proposed model DECLARE.

==> subfiles/conclusions.tex <==
\section{Conclusions}
In this paper, we introduce {\name}, a new stacked approach for automatic medical text simplification and also {\namedata} a new human-annotated medical text simplification dataset. 
In particular, we run multiple baseline models, including a statistical machine translation model, neural machine translation models, and a text summarization model. Besides, three new metrics are designed according to the special requirements of medical language translation. From the experimental results, we find that the stacked approach is the best method in addressing the medical text simplification with both the advantages of the dictionary and translation methods.
And the experiments also prove that the curated dataset {\namedata} is effective benchmark for evaluating the medical text simplification approaches.


==> subfiles/dataset.tex <==
\section{A New Benchmark Dataset}
\fl{First, introduce the motivation: Why we need a new dataset? Second, two steps.}
% To create {\name} data set. There are two major steps: 1) Recognize suitable professional medical sentences, 2) Create the aligned plain customers understandable sentences. We will illustrate the details of the each step in the following two sections.
Despite there are many works~\cite{2014Mining, elhadad2007mining,deleger2008paraphrase,qenam2017text} for constructing mapping relations between professional terms and general descriptions, no works contain aligned simplification sentence results. Without such aligned data, it's also impossible to train our staged simplification pipeline, since it involves context recognition and partially paraphrase tasks. To address the aforementioned challenges, in this paper, also we introduce a human-annotated dataset, named {\namedata}, which aligns professional-to-customer sentences extracted from clinical notes in the MIMIC-III v1.4 database~\cite{johnson2016mimic}. 

There are two key steps when we create the {\namedata} dataset.
%We use two key steps to create such a usable medical language translation dataset.
The first step is to recognize suitable professional medical sentences (named source sentences). The second is to translate those sentences to the aligned plain customer understandable sentences by annotators, which are further checked by experts. We will illustrate the details of each step in the following sub-sections.

\subsection{Source Sentence Collection}
\fl{merge section 2.2.1 and 2.1.2}
\subsubsection{Data Selection}
We first select notes from the NOTEEVENTS table of the MIMIC-III v1.4 dataset\footnote{\url{https://mimic.physionet.org/mimictables/noteevents/}} focusing on the following three sections: (1) History of present illness, (2) Brief summary of hospital course, and (3) Brief hospital course. These three sections contain thoughts and reasoning for the communication between clinicians, which are usually written with professional medical jargon. However it may still contains many plain sentence e.g. \emph{``She now also reports of being hunger.''}. So we further use a heuristic feature-based sentence selection appaorch to avoid selecting thsoe sentences. 
We first tokenize each sentence into a set of words and then use a dictionary-based approach to match medical abbreviations. We also count the number of commonly-used English words within a given list\footnote{\url{https://www.ef.com/wwen/english-resources/english-vocabulary/top-3000-words/}}. 
Based on the length of the sentences (greater than 10), the ratio of medical abbreviations (smaller than 0.5), and the ratio of top-3000 words (greater than 0.1), we can automatically select candidate sentences. 

% \begin{algorithm}[h]
% \caption{Sentence Selection Algorithm} 
% \label{alg:training}
% \small
% \begin{algorithmic}[1]
% \REQUIRE Target sentence $s$, top-3000 word set $T$, medical abbreviation set $A$
% \STATE Tokenize $s$ into words $[w_1,...,w_n]$
% \FOR{$i=1$ to $n$}
% \IF{$w_i\in A$}
% \STATE $abb$ = $abb$ + 1;
% \ENDIF
% \STATE $w_i^{\prime} = lemmatize(w_i)$;E
% \IF{$w_i^{\prime} \notin T$}
% \STATE $unc = unc + 1$;
% \ENDIF
% \ENDFOR
% \IF{$n<10$ or $\frac{unc+abb}{n}>0.5$ or $\frac{unc+abb}{n}<0.1$}
% \STATE \textbf{return} False;
% \ELSE
% \STATE \textbf{return} True;
% \ENDIF
% \end{algorithmic}
% \end{algorithm}

% The sentence selection algorithm is summarized in Algorithm~\ref{alg:training}. For each tokenized word $w_i$, we first check whether it belongs to the medical abbreviation set $A$, and $abb$ in line 4 denotes the current number of medical abbreviations in the target sentence $s$. If $w_i$ is not a medical abbreviation, then we will check whether the lemmatized $w_i$ belongs to the top-3000 word set $T$. $unc$ in line 8 represents the current number of words that are neither medical abbreviations nor commonly-used words. Finally, based on the predefined criteria, the algorithm can automatically decide to keep or remove the target sentence. 

\subsection{Data Annotation}
After we collect a set of source sentences, the next step is to annotate them. 
However, annotating medical sentences is different from creating a parallel bilingual translation corpus. The medical language translation task aims to ``translate'' professional and clinical jargon to layperson-understandable language, which is still from the same language but using different expressions. Besides, annotating bilingual translation data focuses on readability and accuracy. Except for those two perspectives, annotating medical sentences also considers understandability, which is from the perspective of patients or customers. Based on the above guidance, 
%we hire workers to translate the source sentences.
we invited six researchers to annotate the data. All of them are familiar with medical data. For each sentence, there are two extra senior researchers holding the Doctor of Medicine (M.D.) degree to check the annotation quality. For the translated sentences with low quality, senior researchers need to re-translate them.

% Annotation guidance can be found in Figure 1. Annotators are required to (1) replace abbreviations with full terms according to the given dictionary and (2) simplify professional terms to general terms. The dictionary is extracted from the book named “DORLAND’S DICTIONARY of MEDICAL ACRONYMS & ABBREVIATIONS (7th edition)”. If the abbreviations do not exist in the dictionary or the full terms of abbreviations do not match the semantic meanings of the source sentences, the annotators are required to search them on the web. The corresponding abbreviation-full term pair will be added to the dictionary. For a certain abbreviation, since there may be more than one full term, annotators need to pick the best one according to the context. We will add these details to the paper.




The purpose of this work is to create a benchmark for the understandable medical language translation (UMLT) task, which is not only used for training translation models but also for fair evaluation of different approaches. Thus, we set different requirements for workers when annotating the training data and validation/testing data. In general, they use two steps when annotating each source sentence. The first step is to paraphrase the abbreviations with the whole words or phrases. For each abbreviation, there may be several full forms. For example, ``\emph{TLC}'' has two full forms\footnote{\url{https://medical-dictionary.thefreedictionary.com/TLC}}. One is ``\emph{thin-layer chromatography}'', and the other is ``\emph{total lung capacity}''. Therefore, it is important for workers to understand the context in which the abbreviation or term has been used. The second step is to use simple words to replace professorial medical expressions. Take the word ``\emph{hematocrit}''\footnote{\url{https://www.mayoclinic.org/tests-procedures/hematocrit/about/pac-20384728}} as an example, which means the ratio of the volume of red blood cells to the volume of the whole blood. If we use the expression, \emph{``the proportion of red blood cells in the blood''}, it is much understandable for patients compared with directly using professional clinical jargon. An example in Figure~\ref{image:annotation} illustrates the annotating procedure.

When annotating the training data, workers are asked to return the final understandable sentences, i.e., the simplified ones, which will be checked by experts again to guarantee the annotation quality. For validation and testing data, we require workers to return both rephrasing and simplifying forms for each source sentence. 

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{images/annotation.pdf}
\vspace{-0.1in}
\caption{An example of annotating a source sentence by a work using two steps, i.e., rephrasing and simplifying. In the rephrasing step, three abbreviations are replaced by full forms. In the simplifying step, the full form ``nasal cannula'' is replaced by ``tube insertion on nose''.}
\label{image:annotation}
\vspace{-0.15in}
\end{figure}

Note that for all the training, validation, and testing data, there is a special case that we do not need to translate the source sentence. For example, it is easy to understand the sentence ``\emph{He had a set of surveillance blood cultures drawn last week, which were negative.}''. These sentences are extremely useful when training an understandable translation model because they can be considered as important indicators for guiding model learning.  
In the validation and testing data, another special case is that the sentence may not be simplified any more. For example, the source sentence is ``\emph{She also had subjective {SOB} with {CXR} suggesting fluid overload.}'', and the rephrased and simplified sentences are the same, which is ``\emph{She also had subjective [{shortness of breath}] with [{chest x-ray}] suggesting fluid overload.}''.

\begin{table}[!htb]
\centering
\resizebox{0.48\textwidth}{!}{
\footnotesize
\begin{tabular}{|l|c|}
\hline
\# of tokens in the source sentences & 14,780\\\hline
\# of tokens in the target sentences & 14,278\\\hline
\# of overlapped tokens between source \& target  & 12,501\\\hline
Avg. length of the source sentences  & 20.6\\\hline
Avg. length of the target sentences  & 24.0\\\hline
Avg. \# of abbreviations in validation \& testing sets  & 1.2\\\hline
\end{tabular}
}
\vspace{-0.1in}
\caption{{\name} data statistics.}
\label{Table:data}
\vspace{-0.2in}
\end{table}

\subsection{Dataset Statistics}
The {\name} dataset contains 12,801 sentences for training, 1,015 sentences for validation, and 1,016 sentences for testing. Table~\ref{Table:data} shows the statistics of the {\name} dataset, which are different from those of traditional machine translation datasets.
First, the way of annotation is different as we discussed in the previous section. Second, there are a large number of overlapped tokens between source and target sentences, which is also different from traditional machine translation. These differences make our task unique and challenging.  




% \section{The {\name} Dataset}
% To create {\name} data set. There are two major steps: 1) Recognize suitable professional medical sentences, 2) Create the aligned plain customers understandable sentences. We will illustrate the details of the each step in the following two sections.

% \subsection{Source Sentences Collection}
% We used the MIMIC-III v1.4 \cite{} data set to collect the source professional sentences. To be more specific we focus on three parts of the clinical notes: 1) HISTORY OF PRESENT ILLNESS, 2) BRIEF SUMMARY OF HOSPITAL COURSE, 3) BRIEF HOSPITAL COURSE. Because those because sections are generally written for the communications between clinicians. To identify each section, we use regularization method to recognize the section heads and compare the section head with our target list.  
% \junyu{details about the selection of common words and distinguished from the later common words}
% After obtain target sections, we start to select proper candidate sentences. Although those sections contains many professional jargon, still some sentences are plain enough requiring no further explanation. For example, like \emph{"She now also reports of being hunger ."}. To avoid selecting such sentences, we developed a feature-based auto selection methods. We first use the medical diction to recognize medical abbreviations. Then we select 3000 most common English words\footnote{https://www.ef.com/wwen/english-resources/english-vocabulary/top-3000-words/} as base common  words.  For each word in the target sentence we lemmatize the word first, if the lemmatized version is in the base common words set, then we regard it us a common word, otherwise, not a common word. 
% Then we use the ratio of medical abbreviations and uncommon words to decide whether we want the sentence. The detail procedure is defined by the following algorithm:


% Where $n$ is the number of the words, $abb$ is the number the abbreviations and $uncom$ is the number of the uncommon words. Before detect the common words, the target word is lemmatized to obtain Lemmatizatio form. 
% \junyu{add hard examples to case study}
% Notice that, if there is too many uncommon words or abbreviations, we will also reject the sentence, since such sentences are too hard to explain to ordinary users.

% \subsection{Data Annotation}
% After obtain the source sentences, the next step is the annotation. We set different requirements for the annotation of training set and val/test sets. For training set, the taggers are asked to give out the most convenient form of explanation. Each tagger's work will be checked by professional work again to ensure the accuracy. 

% For val/test sets as shown in Table \ref{Tab:valset}, taggers are asked give out the accurate explanation first. If the explanation is still hard to understand, we require the taggers to give out a simpler but less accurate version. \fl{need to give some hard examples. Here, we may need a figure to illustrate how to annotate.}
% \begin{table}[]
% \centering
% \tiny
% \begin{tabular}{|c|c|}
% \hline
% Source:       & The next   day \textcolor{green}{he} received 2 units of \textcolor{red}{PRBC} for \textcolor{red}{hct} of 24.3 .                                                            \\ \hline
% Accurate:     & \makecell{The next day \textcolor{green}{he} received 2   units of \textcolor{red}{PRBC{[}packed red blood cells{]}} \\for \textcolor{red}{hct{[}hematocrit{]}} of 24.3 .}              \\ \hline
% Simple:       & \makecell{The next day \textcolor{green}{he} received 2   units of \textcolor{red}{PRBC{[}packed red blood cells{]}} \\for proportion of red blood cells of   24.3 .}  \\ \hline
% Accurate 2rd: & \makecell{The next day \textcolor{green}{you} received 2   units of \textcolor{red}{PRBC{[}packed red blood cells{]}} \\for \textcolor{red}{hct{[}hematocrit{]}} of 24.3 .}             \\ \hline
% Simple 2rd:   & \makecell{The next day \textcolor{green}{you} received 2   units of \textcolor{red}{PRBC{[}packed red blood cells{]}} \\for proportion of red blood cells of   24.3 .} \\ \hline
% \end{tabular}
% \caption{Examples from the testing/validation set. \textcolor{green}{Green} mark for person,  \textcolor{red}{red} mark for professional abbreviation and under the [] is the corresponding explanation }
% \label{Tab:valset}
% \end{table}
% In addition, we also requires the tagger to provide the annotation in second person. Because in the actual translations, user may prefer a second person version.
% So in total there may be four possible references for one source sentences. Two for different person versions, and two for different simplicity. 
% All versions are used as references in our testing stage for calculating the BLEU score.

% \subsection{Dataset Statistics}
% \fl{I don't think we need to compare with other MT datasets. Add more statistics of our dataset, such as \# ABB, avg. \# ABB in each sentence, and so on. Question: \# of common vocab is not 3000? How many validation data? How many testing data?}
% In total we collected 12,801 sentences for training and 1,015 sentences for validation, 1016 sentences for testing. As we can see in Table \ref{Table:data}, there is a huge difference compared with general machine translation data set. First of all is the difference of the data size. Compared with general translation data set, our data size is much smaller. Thus many state of art giant models in machine translation may not be suitable for this task. Second, there are a lot of intersected words between source and target data. The differences in data size and the huge number of intersected words make our task quite different from the general machine translation task.
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{|c|c|c|}
% \hline
% Train Num      & {\color[HTML]{333333} Val Num}        & Test Num          \\ \hline
% 12,801          & {\color[HTML]{333333} 1,015}           & 1,016              \\ \hline
% Toekn Src      & {\color[HTML]{333333} Token Tar}      & Intersected Token \\ \hline
% 14,780          & {\color[HTML]{333333} 14,278}          & 1,2501             \\ \hline
% Avg Len Src & {\color[HTML]{333333} Avg Len Tar} & Avg Abbreviation           \\ \hline
% 20.597         & 24.0143                               & 1.2               \\ \hline
% \end{tabular}
% \caption{}
% \label{Table:data}
% \end{table}


% \subsection{Dataset Examples}
% In here, we show some of examples from the training and test/validation sets to make a more concrete view of our data set. For testing/validation set, each sentence will have four possible translation targets as described above. The abbreviations marked out using [] notations with the explanation inside the box. 
% \junyu{Better examples and table form}
% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{|c|l|}
% \hline
%                           & \makecell[l]{ Source: Her CXR had what was likely a resolving   pneumonia .}                                                  \\ \cline{2-2} 
% \multirow{-2}{*}{Case 1:} & \makecell[l]{ Target: Her chest x-ray had what was likely a resolving lung infection .}                                       \\ \hline
%                           & \makecell[l]{ Source: The mother is a 28-year-old, gravida 1 , para 0-3 , female .}                                          \\ \cline{2-2} 
% \multirow{-2}{*}{Case 2:} & \makecell[l]{ Target: The mother is a 28-year-old, number of pregnancies 1 , number of   completed pregnancies 0-3 , female} \\ \hline
% \end{tabular}
% \caption{Examples from the training set.}
% \label{Table:trainset}
% \end{table*}

% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{|c|l|}
% \hline
%                           & \makecell[l]{ Source: She was intubated and was resuscitated after 10-22 minutes of PEA arrest .}                                                  \\ \cline{2-2} 
% \multirow{-2}{*}{Case 1:} & \makecell[l]{ 
% Accurate: She was intubated and was waken up after 10-22 minutes of PEA[pulseless electrical activity] arrest .\\
% Simple: She was intubated and was waken up after 10-22 minutes of unresponsive pulse arrest .}                                       \\ \hline
%                           & \makecell[l]{ Source: Upon arrival to the ICU patient is totally CP free .}                                                  \\ \cline{2-2} 
% \multirow{-2}{*}{Case 2:} & \makecell[l]{ 
% Accurate: Upon arrival to the ICU[intensive care unit] patient is totally CP[Cerebral palsy] free .\\
% Simple: Upon arrival to the ICU[intensive care unit] patient is totally motor disability free .}                                       \\ \hline
% \end{tabular}
% \caption{Examples from the testing/validation set.}
% \label{Table:valtestset}
% \end{table*}
% \subsection{Current Inadequacy}
% However, there are still a lot of limitations to our data set. First of all, we remove the tough examples since they are hard for taggers to give out correct answers. In addition, the pre-detection for abbreviation is based on existing dictionary. Although taggers may be able to detect the unmarked abbreviations, it's hard to guarantee. In addition, the readability of training sentences need to further enhance. 


==> subfiles/experiments.tex <==
\section{Experiment}
\fl{add ablation study section to analyze each 'level' of your model design.}
In this section, we conduct experiments on the MedLane dataset to evaluate the performance of {\name}. We will follow the below order to introduce the experiment.
First, is the experimental settings and baselines, then is the evaluation metrics. Finally, the analysis of the experiment results and case study.

\subsection{Dictionary Building}\label{sec:dictionary}
The corpus comes from two sides. The first side is the existing medical abbreviation dictionary\footnote{}. The second side is the from the raw material. During masking the potential subjects that need to be simplified, we also add the tokens that don't include in the dictionary as the potential translation targets and the explanation is obtained from the target sections of the target sentence. For details, please refer to the appendix or the source code.
\subsection{Experimental Settings}
Following methods are used.
Copy means directly copy the input as the answer. It serves as a benchmark for the comparison.
Statistical method Moses\footnote{\url{http://www.statmt.org/moses/manual/manual.pdf}}.
For translation methods, we select, Seq2Seq, and PointerNet, the hidden size is set to 256 for both encoder and decoder by greedy search, the learning rate is set to $1e-3$. We use Adam~\cite{kingma2014adam} as the optimizer. Tokenization is performed using NLTK word tokenizer~\cite{bird2009natural}. 
BERT-MT is as same as the restricted polisher model, expect we directly use it to translate the orgiinal inputs. The learning rate is set to $5e-5$, with warm-up training and the early stop.

For dictionary based method, we use the professional medical dictionary to replace the found terms in an input sentence, if there are multiple answers, we randomly select one as the result. We do not use the full-size dictionary that includes the potential explanation learned from the raw material. Since, it will introduce extra noises, without the position selection model, the performance can be greatly influenced.

Not all related methods are selected, due to the problem specialty. Most related works address a different setting, for example break a long sentence into simple sentences. Or perform simplification on UMLS concepts. Here, our focus is on the abbreviations/terminology simplification.


For {\name}, Locker Module, a bert model pre-trained on PubMedical~\cite{} text is applied to perform token level classification, with the learning rate $5e-5$ and 5 training epochs. Early stop is applied by checking the training loss on the validation set.

For neural interpreter, we apply the same setting from the \cite{zhang2020dcmn+}. The max size of the answers is set to 8. The maximum length of the input sentence is set to 64 during training. Learning rate is set to $5e-5$ with 10 epochs. Early stop is adopted.

For restricted polisher, $5e-5$ learning rate with the warm-up training method as the BERT-MT. Batch size is set to 30 and using BLEU to perform early stop. The maximum length of the input sentence is set to 128.

\subsection{Evaluation Metrics}
\begin{figure}[!htb]\small
 \centering
% \vspace{-0.05in}
\begin{minipage}[h]{0.4\textwidth}
\fbox{
\parbox{\textwidth}{
{\tt{
\textbf{Source}: vascular saw the \textcolor{blue}{pt} and did not feel that there was an acute need for an invasive procedure .\\
\textbf{Target}: vascular saw the \textcolor{red}{patient} and did not feel that there was an acute need for an invasive procedure .
}}
}
}
\end{minipage}
 \vspace{-0.1in}
\caption{Example of the failure of existing metrics.}\label{fig:example}
 \vspace{-0.15in}
\end{figure}
We select BLEU~\cite{papineni2002bleu}, METEOR~\cite{lavie2007meteor}, ROUGE-L~\cite{lin2004rouge}, CIDEr~\cite{vedantam2015cider} scores that are generally used to evaluate the machine translation tasks. 
%Besides those methods, we select \emph{Hit Ration (HIT)}, \emph{Common Word Ration (CWR)}, \emph{Aggregation Score (AScore)} methods from \cite{} to address the special requirements of the medical text simplification.
\emph{HIT} evaluates the simplification accuracy of the abbreviations and professional terms. \emph{CWR} is a used to evaluate the simplicity of the translated sentences. \emph{Ascore} serves as an overall evaluation of the BLEU, HIT, and CWR scores.
\subsubsection{Task-specific Metrics}
Since our task is different from traditional machine translation tasks, directly applying existing evaluation metrics cannot fairly evaluate the performance of different models. Here, we use an example in Figure~\ref{fig:example} to demonstrate the failure of existing evaluation metrics, such as BLEU score. If we directly copy the original source sentence as the answer, a very high BLEU score can be obtained, which is 0.85. However, the critical term ``\emph{pt}'' is not translated. Without translating this term, patients or customers may not totally understand the meaning of this sentence. Thus, it is necessary to design task-specific metrics. 

$\bullet$ \emph{Hit Ration (HIT)}. A key challenge of medical language translation is to translate professional medical jargon to layperson-understandable words. Let $N_p$ denote the number of professional medical terms in a source sentence and $N_t$ be the number of correctly translated terms in the target. We then have the HIT ration, which is $HIT = \frac{N_t}{N_p}$.
    
$\bullet$ \emph{Common Word Ration (CWR)}. To evaluate the simplicity of the translated sentences, we calculate the common word ratio for each output sentence. We first lemmatize each word of the output. If the lemmatized form is in the top-3000 commonly-used English words, then it is a common word. Otherwise, it is not a common word. Let $N_c$ denote the number of common words in the translated sentence and $N$ represents the length of the translated sentence. The common word ratio score is $CWR=\frac{N_c}{N}$.
    
$\bullet$ \emph{Aggregation Score (AScore)}. The quality of the translated sentences is not only decided by the readability (BLEU) but also related to the correctness (HIT) and simplicity (CWR). Among these three perspectives, readability and correctness should be more important than simplicity. Thus, we design a new score to model them at the same time, which is
    \begin{equation*}
        Ascore = \frac{1+\alpha^2+\beta^2}{\frac{\alpha^2}{BLEU} + \frac{\beta^2}{HIT} + \frac{1}{CWR}},
    \end{equation*}
    where $\alpha$ and $\beta$ are parameters for controlling the importance of BLEU and HIT scores. If any of the three metrics is 0, then it will be added to a very small number such as $10^{-8}$ to avoid AScore to be 0. We take $\alpha=2$ and $\beta=1.5$ in our experiments.

\subsection{Experimental Results}
\noindent\textbf{Statistical Performance Analysis}.
Table~\ref{Table:exp} shows the statistical experimental results on all the metrics. {\name} family outperforms the remaining baselines on the most of evaluation metrics.

The Dictionary method is the most simple metric in terms of the parameters. And it also has the worst performance. The major reason is the multi choice problem and the context problem. Due to the context, a term can be a terminology or not. And the corresponding answers are also different under different setting. Dictionary approach cannot manage the above two problems.

The statistical method Moses has a better performance. As a traditional language translation model, it has the ability of recognizing the context. Yet, the ability of finding ans simplifying the terminologies is poor, according to the HIT score and CWR score.

For neural machine translation methods, including Seq2Seq variants, PointerNet, and PMBERT MT. We can see a significant improvement on the HIT and CWR scores. But in the meanwhile, we can find that their BLEU scores are also lower compared to the simple copy. Thus, it means that those methods also change many unnecessary parts during the simplification. Under the setting of the medical simplification, it's dangerous. For example, it may change some time or location information and cause a wrong understanding. 

For {\name} family, the neural interpreter output has the highest scores on the most metrics. And if we directly applied a translation layer, there will be a great drop on the BLEU scores. Similar drawbacks of the translation methods appear again. Unnecessary changes are made. But with the partial translation setting, this problem is greatly reduced and the CWR score is improved too. Although from the scores, it seems that full method with the partial translation is still worse than the pure neural interpreter output, we will prove with the case study that such efforts are valued in the aspect of fluency and readability.
\\

\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Model}            & \textbf{BLEU-1}                         & \textbf{BLEU-2}  & \textbf{BLEU-3}  & \textbf{BLEU-4}  & \textbf{BLEU} & \textbf{METEOR} & \textbf{ROUGE-L} & \textbf{CIDEr}  & \textbf{HIT}    & \textbf{CWR}    & \textbf{AScore}  \\ \hline
Copy       & 0.7898                        & 0.7495 & 0.7147 & 0.6826 & 0.7342 & 0.4601 & 0.8496 & 5.9432 & 0.5400 & 0.7001 & 0.6323 \\ \hline
Moses      & 0.7880                       & 0.7130 & 0.6530 & 0.6016 & 0.6889 & 0.4237 & 0.8188 & 5.1046 & 0.6823 & 0.7543 & 0.6859 \\ \hline
Dictionary & 0.7158                       & 0.6364 & 0.5684 & 0.5076 & 0.6070 & 0.3933 & 0.7308 & 4.2037 & 0.5572 & 0.6407 & 0.5948 \\ \hline
Seq2seq    & 0.7136                       & 0.6322 & 0.5969 & 0.5160 & 0.6147 & 0.3533 & 0.7609 & 4.1299 & 0.7388 & 0.7980 & 0.6648 \\ \hline
Seq2seq-   & 0.5066                       & 0.3315 & 0.2373 & 0.1787 & 0.3135 & 0.1859 & 0.4948 & 1.2670 & 0.6427 & 0.8367 & 0.4070 \\ \hline
Seq2seq-S  & 0.7180                       & 0.6386 & 0.5778 & 0.5267 & 0.6153 & 0.3604 & 0.7683 & 4.2635 & 0.7331 & 0.7953 & 0.6630 \\ \hline
PointerNet & 0.6870                       & 0.5904 & 0.5158 & 0.4541 & 0.5618 & 0.3338 & 0.7285 & 3.9458 & 0.6414 & 0.7555 & 0.5949 \\ \hline
BERT-MT  & 0.8003                       & 0.7428 & 0.6952 & 0.6531 & 0.7228 & 0.4566 & 0.8218 & 5.3293 & 0.7808 & 0.7358 & 0.7417 \\ \hline
%SSimp 1+2   & 0.8840                      & 0.8557 & 0.8304 & 0.8064 & 0.8441 & 0.5495 & 0.9096 & 7.0476 & 0.8134 & 0.7250 & 0.8161 \\ \hline
%SSimp 1+2+3 Full   & 0.8052               & 0.7498 & 0.7093 & 0.6621 & 0.7302 & 0.4637 & 0.8301 & 5.4110 & 0.7833 & 0.7343 & 0.7465 \\ \hline
SSimp & 0.8728               & 0.8392 & 0.8103 & 0.7835 & 0.8265 & 0.5319 & 0.8940 & 6.7700 & 0.7762 & 0.7312 & 0.7962 \\ \hline
%STS  & 0.8028 & 0.7524 & 0.7103 & 0.6722 & 0.7344 & 0.4604 & 0.8266 & 5.6442 & 0.5734 & 0.7092 & 0.6725 \\ \hline
%Rank    & 1 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 1 & 6 & 1\\\hline
\end{tabular}
}
\vspace{-0.1in}
\caption{Performance evaluation of all the baselines with eleven metrics.}
\label{Table:exp}
\vspace{-0.1in}
\end{table*}
\noindent\textbf{Case Study}
Despite from the statistic standards the performance of the completed three stage method worse than the two stage method, but it doesn't mean the actual performance of the completed method is worse. Thus we select some examples from the test result to perform case to case study to show the necessity of the polishing step.

As shown in Table~\ref{Table:case1}. Partial translation method accurately recognize and mark out the key translation section. Although it also changes the other parts of the input, but with the help the special mask separation, the mistakes can be fixed. Thus, the final result is perfect. Only the complete process is able to give out a further simplified result.
And the reason for the lower scores is majorly due to the grammar mistakes of the training data. E.g. translate the word "\emph{nonpassage}" into "\emph{nonpecge}", which is readable for human, but wrong answer for the machine.

\noindent\textbf{Failure Cases}
\begin{table}[!htb]
\small
\centering
\begin{tabular}{|l|l|}
\hline
1 & nonpassage -\textgreater nonpecge                         \\ \hline
2 & last name (if) -\textgreater last name ((()               \\ \hline
3 & hemodynamically -\textgreater blood dynamics              \\ \hline
4 & nstemi/cad -\textgreater heart attack attack/heart attack \\ \hline
5 & hearts failure -\textgreater heart failure                \\ \hline
6 & name10 907 ua -\textgreater name10 907                    \\ \hline
\end{tabular}
\vspace{-0.1in}
\caption{Example “failures” of the restricted polisher.}
\label{Table:exp_failure}
\vspace{-0.1in}
\end{table}
We also collect "failed examples" in the Table~\ref{Table:exp_failure} of the restricted polisher to discover the inner logic.
The left part is the "correct" version and the right part next to the "-\textgreater" is the output of the restricted polisher. For cases 1,2,5,6, the outputs of the restricted polisher are almost equal to the correct answers for a human reader.
For cases 3, 4, the annotations did not explain the professional terms. Although there are slight mistakes for the output the polisher, the polished versions are closer to the lay language. 

\noindent\textbf{Human Evaluation}

\smallskip
\noindent\textbf{Parameter Analysis}.
In the proposed new metric AScore, there are two key parameters $\alpha$ and $\beta$. Figure~\ref{image:parameter} shows the values of AScore with regard to the changes of $\alpha$ and $\beta$. We can observe that given a fixed $\alpha$, the values of AScore increase with the increase of $\beta$. When we fix the value of $\beta$, the values of AScore will decrease with the increase of $\alpha$. The values of AScore are in the range [BLEU, HIT]. Thus, AScore is a trade-off between readability (BLEU), correctness (HIT), and simplicity (CWR). 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{images/medlan_plot.pdf}
\vspace{-0.1in}
\caption{Ascore changes regrading $\alpha$ and $\beta$.}
\label{image:parameter}
\vspace{-0.1in}
\end{figure}

\begin{table*}[]
\small
\begin{tabular}{|l|l|}
\hline
{\color[HTML]{333333} In} & encourage/assist with po intake and give supplements at minimum of 3 times daily .                                            \\ \hline
Tar 1                     & encourage/assist with oral intake and give supplements at minimum of 3 times daily .                                      \\ \hline
Tar 2 further simplified  & encourage/assist with by mouth intake and give supplements at minimum of 3 times daily .                                      \\ \hline
L 2                        & encourage/assist with by mouth, that is, orally (from latin per os) intake and give supplements at \\
&minimum of 3 times daily . \\ \hline
L 3 Full                   & rein / assist with by mouth intake and give supplements at at of 3 times daily .                                              \\ \hline
L 3 Partial Raw           & tolerate / assist with {[}MASK{]} by mouth {[}MASK{]} intake and give supplements at of times times daily .                   \\ \hline
L 3 Partial               & encourage/assist with by mouth intake and give supplements at minimum of 3 times daily .                                      \\ \hline
\end{tabular}
\vspace{-0.1in}
\caption{Case study.}
\label{Table:case1}
\vspace{-0.2in}
\end{table*}
 

==> subfiles/introduction.tex <==
\section{Introduction}
The increasing accessibility of technology information makes patients have more opportunities to understand their own health situation and enable more communications between patients and doctors.
However, such communication relies on the additional efforts of the clinicians. The professional jargon and abbreviation make it impossible for ordinary user to directly communicate. 
The lack of proper communication may result a tense doctor-patient relationship~\cite{ha2010doctor}.


Therefore, there is a great need for automatically simplifying professional clinical language to layperson-understandable language.

To address the problem, many approaches are proposed.
The first nature idea is to use expert dictionaries to map the key terms into ordinary language~\cite{kandula2010semantic,zeng2006exploring,zeng2007making}. Further, we can add language pattern to improve the translation quality...
Although some similar work~\cite{cao2020expertise, guo2020automated} also address this issue, they are based on a totally different setting.

% \yaqing{Recently, researchers cast the medical language understanding task as a neural machine translation task~\cite{weng2019unsupervised}. However, due to the lack of aligned sentences, the existing studies usually treat the medical language understanding task as an unsupervised translation task and cannot obtain an accurate, usable, and reliable translation model. To further improve the progress of medical language understanding task, it is necessary to construct a high-quality and large-scale aligned sentence dataset.}

To address the aforementioned challenges, in this paper, we introduce a new stacked medical language simplification system, named {\name}. Based on the above mentioned problem, the simplification is structured into three levels. Level one aims at selecting potential intricate words. Level two focuses on using a professional dictionary and context to select best-matched candidate answers. The final step severs as an insurance to further improve or correct the simplifications results from the first two levels. The three levels of model are trained as a whole. We also introduce a human-annotated dataset, named {\namedata}, which aligns professional-to-customer sentences extracted from clinical notes in the MIMIC-III v1.4 database~\cite{johnson2016mimic}. 
To sum up, our major contributions are listed as follows:

%$\bullet$ \textbf{A New Dataset}. To the best of our knowledge, {\name} is the first new, publicly available, human-annotated dataset for dealing with the understandable medical language translation task (UMLT), which consists of 12,801 training samples, 1,015 validation samples, and 1,016 testing samples.

\textcolor{red}{$\bullet$ \textbf{A New Dataset}. To the best of our knowledge, {\name} is the the first new medical text simplification dataset with both term-level normalization and translation level evaluation, which consists of 12,801 training samples, 1,015 validation samples, and 1,016 testing samples.}

$\bullet$ \textbf{Novel Measurements}. Different from bilingual translation tasks, our task is to translate professional medical jargon to layperson-understandable language. We not only require the translated results readable but also accurate and easily understandable. Thus, we design three new yet general evaluation metrics, which can also be used for other tasks such as medical report generation.

$\bullet$ \textbf{A Safe Simplification System}. The simplification process is strictly limited to avoid any out of domain or miss translation.Final a limited rephrase layer is added that makes system can correct the previous failures and make the language more fluent.



==> subfiles/models.tex <==
\section{Method}
\begin{figure*}[h]
\vspace{-0.1in}
\centering
\includegraphics[width=1.0\textwidth]{images/model_alpha.pdf}
\vspace{-0.1in}
\caption{Overview of {\name} model. (source file: /junyu/emnlp2021)}
\label{image:model}
\vspace{-0.19in}
\end{figure*}
\fl{You need to clearly mention your motivations. Since there are several challenges, you need to design such a model. The section names from level 1 to 3 are not meaningful. Rename them! Similarly, talk more motivations for each section.}
Each medical sentence can be regarded as a ordered sequence of different tokens.
Thus the simplification task can be formalized as a sequence generation task.
Let $W = [w_1,w_2,···,w_n]$ denotes the tokenized professional medical sentence $s$. 
The output is also a sentence $Y = [y_1,y_2,···,y_m]$
Some special tokens will be added to help the model process the information, which we will describe it in the sub-sections. 

To handle the task, we propose a staged simplification model {\name} dividing the task into three phases as illustrated in Figure.~\ref{image:model}.
The lock stage aims at digging out possible phrases that need to be simplified. So the simplification process won't disturb the parts that doesn't need to be changed.
After locking the target, we apply a modified neural dictionary approach to find accurate explanation from a professional medical term dictionary. Final a limited rephrase module is introduced to correct possible errors and insure fluency. 

\subsection{Locker Module}
Giving an input sentence, the first priority is to find out the tokens that need to be modified. So we can concentrate on the target information and prevent modification of the protected information. Hence, we propose to the lock the target information via an sequence classification model. Using the classification result to indicate whether the current token needs to be modified. Let $\mbox{LM}_{p}$ denotes the language model that is used to lock targets. 
\begin{equation}
    P = \mbox{LM}_{p}([w_1,w_2,···,w_n])
\end{equation}
Where $P=[p_1,p_2,...,p_m]$. $p_i$ stands for the possibility that $ith$ token needs to be simplified.
$Loss_{p}$ is the loss function of the level one module. Where $\hat{p_i}$ is the ground truth. For the generation of the ground-truth please refer to the Appendix algorithm~\ref{}.
The final training loss of the Locker is like this:
\begin{equation}
    Loss_{p} = -\frac{1}{n}\sum_{i=1...m}\hat{p_i}\mbox{log}(p_i)+(1-\hat{p_i})\mbox{log}(1-p_i)
\end{equation}

\subsection{Neural Interpreter}
After locking the target, the next step is to select proper explanations from the mapping dictionary. The previous methods~\cite{Kang2016A, Weng2018Mapping, kandula2010semantic} generally choose the answer that has the closet semantic distance. It works fine for some medical terms, but can not deal with the abbreviations. Based on the context, an abbreviation can have multiple answers and totally different in semantic level. Thus we need a new method that can choose answer based on the context information. The recent question answer (QA) technology shows a great capability in solving many problems that are hard to define. We borrow ideas from the question answer (QA)~\cite{zhang2020dcmn+} research to propose the neural interpreter module. We regard the text sentence as the context the corresponding dictionary explanations as the possible answers. The professional terms are regarded as the questions. So we can achieve a context based explanation selection. 
\begin{equation}
    Q = \mbox{QA}(W^{'}, T, A)
\end{equation}
Where $T$ is the target term, $A=[a_1,a_2,...,a_l]$ is the group of possible explanations.
$W^{'}=[w_1,\mbox{[MASK]},w_3,···,w_n]$ is the processed input sentence. We use the [MASK] token to indicate the location of the target term.
$Q=[q_1, q_2, ..., q_l]$ is the probabilities that $ith$ explanation is the correct answer.
$QA$ is our selected QA model.
In the situations that the selected targets are not in the dictionary $D$, the neural interpreter procedure will not be performed.
If there are multiple targets.
The targets will be broken up into different individual QA question. 
$Loss_{q}$ is the loss function of the level two module. Where $q_i$ is the predicted probability of the ground truth answer.
\begin{equation}
    Loss_{q} = -\frac{1}{m}\sum_{i=1...m}\mbox{log}(q_i)
\end{equation}

\subsection{Restricted Polisher}
\begin{figure}[h]
\vspace{-0.1in}
\centering
\includegraphics[width=0.3\textwidth]{images/pmbert.pdf}
\vspace{-0.1in}
\caption{Overview of the level 3 model. It can be also used to directly preform the simplification.}
\label{image:BERT}
\vspace{-0.15in}
\end{figure}

With the previous two steps, we can precisely transfer the abbreviations and complicated terms into the more general terms. However, such replacements are mechanical and not fluent enough on some extreme cases. Thus, we need to further polish the results. But directly apply a paraphrase model to polish the sentence will also introduce many unnecessary modification. To solve this problem, we regard the final task as a partial translation task to translate the previous output to the final desired output.  Partial means we only translate a part of the input sentence.

Let $\tilde{W}=[\tilde{w}_1, \tilde{w}_2, \cdots, \tilde{w}_n]$ denotes the tokenized simplified output of the neural interpreter $\mathbf{s}$.
Let $\hat{Y}=[\hat{y}_1, \hat{y}_2, \cdots, \hat{y}_m]$ denotes the tokenized final target output $\mathbf{t}$. 
For each training pair, we use the [MASK] token to distinguish the parts that requires further translation. Thus, the target of the translation model will be like $[\hat{y}_1, \mbox{[MASK]}, \hat{y}_2, \mbox{[MASK]},\cdots, \hat{y}_m]$, if $y_2$ is the required part.
\begin{equation}
    Loss_{t} = -\frac{1}{m}\sum_{i=1...m}\mbox{log}(p_{\hat{y}_i})
\end{equation}
where $p_{y_i}$ is the probability of token $\hat{y}_i$ at position $i$.

For example if the $\mathbf{s}$ is \emph{"electroencephalogram pattern and clinical exam."} and $\mathbf{t}$ is \emph{"brain electrical activity detection pattern and clinical exam."}, then the desired output will be \emph{"[MASK] brain electrical activity detection [MASK] pattern and clinical exam."} 
By such special setting, we can let the model learns to distinguish the required translation part. On evaluation stage, we only keep the changes between the [MASK] tokens and keep the other parts as same as the inputs. Although it may looks like a redundant approach. But due to the instability of the translation model, many parts that don't require translation will be modified by the translation model. We have proved it on our experiment section. Thus, this step is necessary.

\subsection{Stage Training}
Three modules can be trained together using the ground-truth as the inputs for training first.
\begin{equation}
    Loss_{All} = Loss_{p} + Loss_{q} + Loss_{t}
\end{equation}
Thus, we directly use the $Loss_{All}$ to update three models during the training.
At he evaluation stage, they are performed following a sequence order.






==> subfiles/relatedwork.tex <==
\section{Related Work}
\subsection{Medical Text Simplification}
Due to the great potential value of medical text simplification. Many approaches are proposed.
They can be categorized into three types. 
The first type is is the dictionary-based approach that relies on using the expert-curated medical dictionary to simplify the professional medical sentences~\cite{kandula2010semantic, zeng2006exploring, zeng2007making}. Dictionary approach is highly reliable, yet cannot manage the case of polysemant, a term can have multiple correct explanations under different cases.
And there is only a small amount of medical acronyms/abbreviations normalization data~\cite{elhadad2013share}. Yet it only focuses on choosing the right answer from the possible explanations, doesn't include finding the terms.
There are also pattern-based approaches that aim to discover pairs of professional and consumer terms from the raw training corpus~\cite{2014Mining, elhadad2007mining,deleger2008paraphrase,qenam2017text}. But it's closer to a method for extracting potential dictionary. The ultimate aim is to generate a proper translation dictionary instead of how to better utilize the dictionary. Similarly some works try to create aligned sentences from online materials pairs like Wikipedia and SimpleWikipedia to automatically create aligned training pairs~\cite{van2019evaluating, adduru2018towards}.
However the problem becomes a paraphrasing problem under such settings, similar to translation works. The actual mapping between key terms and simplified explanation cannot be found. The key problem is that the language style and approximate equivalence is allowed~\cite{bhagat2013paraphrase}, but the requirement of accuracy of medical terms make us hard to find whether the approximate equivalence is acceptable under a specific context. 

Researchers also try to borrow ideas from machine translation, like aligning word embeddings between professional terms and daily expressions to achieve the translation~\cite{Kang2016A, Weng2018Mapping}. Or further using back translation procedures to improve the simplification results under unsupervised conditions~\cite{weng2019unsupervised}. 
Despite those methods don't require aligned sentence pairs, their translation accuracy is hard to guarantee. For medical terms, a wrong simplification may cause many potential damage. For general language translation, there is no such concerns. 
Similarly, the work of \cite{cao2020expertise} borrows idea from the text style translation.
The setting is similar to the unsupervised learning without parallel sentence pairs.
During the translation procedure, many unrelated information may be changed.
Thus it may not be suitable for the simplification of some medical reports that requires high accuracy. The work of~\cite{guo2020automated} as lo address the similar question but its major focus is the text summarization of the biomedical articles.

\subsection{Medical Natural Language Processing}
The MIMIC-III database~\cite{johnson2016mimic} contains de-identified data from 58,976 ICU patient admissions, which includes several types of medical information such as demographics, medications, clinical notes, and so on. Most existing works mainly leverage medical codes and biosignals for disease detection~\cite{ma2018kame}, readmission prediction~\cite{du2020joint}, and so on. There are some studies focusing on using the clinical notes for automated ICD coding~\cite{li2020icd,xie2018neural,cao2020hypercore}, natural language inference~\cite{2018Lessons} and unsupervised medical language translation~\cite{weng2019unsupervised}. 

National NLP Clinical Challenges (n2c2)\footnote{\url{https://portal.dbmi.hms.harvard.edu/projects/n2c2-nlp/}}  (the original i2b2 NLP datasets) provide unstructured notes from the Research Patient Data Repository at Partners Healthcare System in Boston. The challenges include clinical trial cohort selection, adverse drug events and medication extraction, clinical concept normalization, clinical semantic textual similarity, etc., which are different from our task. 

Though the MIMIC-III and n2c2 datasets contain clinical notes, none of them provides publicly available human-annotated and aligned data used for translating professional clinical jargon to layperson-understandable language. Thus, the {\name} dataset is unique yet necessary. 

\subsection{Acronyms/Abbreviations Normalization}
There is a medical acronyms/abbreviations normalization dataset from the Task 2 of the 2013 CLEF eHealth workshop \cite{elhadad2013share}, which focuses on the completion of abbreviations -- assigning acronyms and abbreviations to concept unique identifiers (CUIs). The dataset is designed for a \textbf{classification} problem. 
However, our dataset supports a \textbf{translation} task that requires automatically identifying and translating hard medical words. The annotators are also required to give out a more readable version if translating the abbreviations is not enough, which leads to rewriting of the sentences.
Besides, in our task, the acronyms/abbreviations are not limited to phrases, but they can be any forms of the language structures as long as the annotators believe that they are hard to understand for the ordinary customers. Table \ref{Tab:CompData} summarizes the major differences between these datasets.
\begin{table}[h]
\centering
\small
\begin{tabular}{|l|c|c|}
\hline
Language Structure  & MedLane   & CLEF \\\hline
Abbreviation     &\checkmark & \checkmark \\\hline
Acronyms         & \checkmark& \checkmark \\\hline
Complex Phrase   &\checkmark & $\times$ \\\hline         
Sentence Polish  &\checkmark & $\times$ \\\hline
\end{tabular}
\vspace{-0.1in}
\caption{Dataset comparison.}
\label{Tab:CompData}
\vspace{-0.2in}
\end{table}
